EDEN: Empathetic Dialogues for English learning

Dialogue systems have been used as conversation partners in English learning, but few have studied whether these systems improve learning outcomes. Student passion and perseverance, or grit, has been associated with language learning success. Recent work establishes that as students perceive their English teachers to be more supportive, their grit improves. Hypothesizing that the same pattern applies to English-teaching chatbots, we create EDEN, a robust open-domain chatbot for spoken conversation practice that provides empathetic feedback. To construct EDEN, we first train a specialized spoken utterance grammar correction model and a high-quality social chit-chat conversation model. We then conduct a preliminary user study with a variety of strategies for empathetic feedback. Our experiment suggests that using adaptive empathetic feedback leads to higher perceived affective support. Furthermore, elements of perceived affective support positively correlate with student grit.

==> convo_examples.tex <==
\noindent\rule{6cm}{0.4pt}

\noindent \textbf{Conversation Segment:}
\begin{enumerate}
    \item To be honest, I don't want to live on another planet because I think the earth is comfortable and it is suitable for us.
    \item A little. I have some knowledge about the moon and the moon. 
    \item When I was a student in primary school, I went to... I often go to a picnic with my friends. 
\end{enumerate}

\noindent \textbf{Zeroshot:} You have a good grasp of the topic and can express your thoughts clearly. However, you can work on your fluency and pronunciation to make your speech more natural and easy to understand. For example, you can practice speaking more slowly and enunciating your words clearly. Also, try to listen to native speakers and imitate their pronunciation to improve your own. Keep up the good work!

\noindent \textbf{Optimized:} You have a good understanding of the topic and can express your thoughts clearly, which is great! However, you can work on your grammar and sentence structure to make your speech more fluent and natural. For example, instead of saying ``I went to... I often go to a picnic'', you can say ``I used to go on picnics with my friends when I was a student in primary school.'' This will make your sentence more grammatically correct and sound more natural. Keep practicing and you will improve in no time!

\noindent \textbf{Rewrite:} You've got a good handle on the topic and express yourself clearly, which is awesome! Just tweak your grammar and sentence structure for a smoother and more natural flow. For example, instead of saying ``I went to... I often go to a picnic,'' try ``I used to go on picnics with my friends back in primary school.'' Keep at it, and you'll get even better in no time!

\noindent\rule{6cm}{0.4pt}

\noindent \textbf{Conversation Segment:}
\begin{enumerate}
    \item Well, probably like less diet, less fat tissues would really be beneficial to your health and to your general functions.
    \item What's the word again? I've never heard of it. Could you explain the terminology to me?
    \item Okay, that sounds... Well, I'm asking you the word you're talking about the triple action capillates. Yeah, but what's that?
\end{enumerate}

\noindent \textbf{Zeroshot:} You have a good understanding of vocabulary and sentence structure, but you may need to work on your pronunciation and listening skills. For example, when you didn't understand the word ``capillates,'' you asked for clarification, which is great. To improve, try practicing speaking and listening to English more often. Keep asking for clarification when needed, and you'll continue to improve.

\noindent \textbf{Optimized:} You have a good understanding of the topic and can express your thoughts clearly, which is great! However, you can work on your vocabulary and pronunciation to improve your fluency. For example, instead of saying ``less diet,'' you can say ``a healthier diet'' and instead of saying ``capillates,'' you can say ``capillaries.'' Keep practicing and expanding your vocabulary to improve your skills.

\noindent \textbf{Rewrite:} You've got a good grasp of the topic and can explain things clearly, which is awesome! Just work on your vocab and pronunciation for smoother conversation. Try swapping ``less diet'' for ``healthier diet'' and ``capillates'' for ``capillaries.'' Keep at it and keep expanding your vocab to get even better!

\noindent\rule{6cm}{0.4pt}

\noindent \textbf{Conversation Segment:}
\begin{enumerate}
    \item Hmm, actually it depends. If I'm concentrating on the things that I'm interested in, I won't feel bored. But if the things just go so embarrassed or so boring, I will distract by something else. And another situation is that I may fall asleep. 
    \item Well, I actually do not have a memory of that. Because I think sitting on the floors may be the things that the boys do. And however, you know, I'm a girl who likes a tiny and quiet place to sit.  
    \item Of course, while speaking of a person with these strong impression, I would say that was my Chinese teacher in my primary school. I remember she taught us in my fifth grade. At my first sight, she looked really irradible, which made me have the feeling of this teacher is the person you can't get along well with. So I always keep the distance with her. However, what upset me the most was right there. These schools always don't allow the students to bring any entertainment things. I was just a kid, so I bought some comics to my friend as well as some classmates and spread it. Well, the comics are really interesting. After my Chinese teacher, who is also my class class teacher, knew that she just threw it out of my classroom window in front of all my classmates. And that was really embarrassing. So that memory kept kept a long time in my mind and I don't really like that teacher. Even now, I can still remember her with not really good memories.
\end{enumerate}

\noindent \textbf{Zeroshot:} You're doing great in English, you can express yourself well and your thoughts are clear. But you can work on your pronunciation and intonation to make your speech more engaging and natural. Try practicing in front of a mirror or recording yourself to identify areas for improvement. Keep it up!

\noindent \textbf{Optimized:} You have a good understanding of the topic and can express your thoughts clearly, which is great! However, you can work on your grammar and sentence structure to make your speech more fluent and natural. For example, instead of saying "I remember she taught us in my fifth grade", you can say "I remember she taught us when I was in fifth grade." Also, try to use more descriptive words to make your story more engaging. Keep practicing and you will continue to improve!

\noindent \textbf{Rewrite:} You've got a good grasp of the topic and express yourself clearly, awesome! Just tweak your grammar and sentence structure for a smoother flow. For example, instead of saying "I remember she taught us in my fifth grade," you could say "I remember she taught us when I was in fifth grade." Keep practicing, and you'll keep improving!

\noindent\rule{6cm}{0.4pt}

\noindent \textbf{Conversation Segment:}
\begin{enumerate}
    \item People are often willing to get to know new people in various situations. Firstly, when individuals join new social or professional environments, such as starting a new job or moving to a new city, they are more open to meeting new people as they seek to establish social connections and build a support network. Secondly,
    \item People go to various places to meet new people and expand their social circles. One common place is social events and gatherings such as parties, social clubs and community events. These provide opportunities for individuals to interact with others who share similar interests or are part of the same community.
    \item Studying a conversation can be approached in various ways depending on the context and the individuals involved. One common way is through initiating a topic of mutual interest. This could involve asking open-ended questions or making observations about the current situation. For example, at a social gathering, one might start a conversation by commenting on the events, complimenting someone's attire, or discussing a shared hobby.
\end{enumerate}

\noindent \textbf{Zeroshot:} You're great at starting conversations and finding common interests with others, which is a valuable skill in making new connections. However, you can work on being more confident and assertive in your approach, as well as actively listening and asking follow-up questions to keep the conversation going. For example, instead of just commenting on the events, try asking others about their experiences or opinions. This will show your interest and help you build deeper connections with people.

\noindent \textbf{Optimized:} You have a good understanding of the topic and can explain it clearly. However, you can work on your pronunciation and intonation to make your speech more engaging and natural. For example, try to vary your tone and emphasize important words to make your speech more interesting. Keep practicing and you will continue to improve!

\noindent \textbf{Rewrite:} You've got a good grip on the topic and explain it well. To spice up your speech, try varying your tone and emphasizing important words. Keep practicing, and you'll keep getting better!

\noindent\rule{6cm}{0.4pt}

\noindent \textbf{Conversation Segment:}
\begin{enumerate}
    \item Well, I'm afraid that I can't give you the straight answer. But in the city where I live now, the weather is always raining because it's located in the southeastern part of China and it's also close to the sea. Sometimes I like to stay in the sunny days because I really like the moment when I read some books in the afternoon in the sunny days.
    \item Well, there are some different kinds of styles in terms of weather situations in my hometown. For instance, in spring, the air is mild and fresh. In summer, the weather is so hot. In autumn, the weather started to become a little cold compared with the weather in summer. In winter, the weather in my hometown is quite cold.
    \item Well, I'm afraid that I can't give you the straight answer. This mainly depends on different situations. When the weather is so dry, so when it's raining, I really like the rainy days. On the contrary, as I mentioned before, I really like the time when I spent in the sunny days like reading a book when I felt very tired.
\end{enumerate}

\noindent \textbf{Zeroshot:} Hey there! Your pronunciation and intonation are on point, making it easy for me to understand you. But to make your speech more interesting, try using different words and sentence structures. For example, instead of saying "I really like", you can say "I'm fond of" or "I'm a big fan of". Also, use more descriptive adjectives like "scorching" or "sweltering" to paint a clearer picture. Keep practicing and you'll see improvement in no time!

\noindent \textbf{Optimized:} You have a good understanding of different weather situations and can describe them clearly, which is great! However, you can work on your grammar and sentence structure to make your speech more fluent and natural. For example, instead of saying "I really like the time when I spent in the sunny days", you can say "I really enjoy spending time in the sunny days." Keep practicing and you will continue to improve!

\noindent \textbf{Rewrite:} You're good at understanding different weather situations and describing them clearly, that's awesome! Just work on grammar and sentence structure to make your speech flow better. For example, say "I love spending time on sunny days" instead of "I really like the time when I spent in the sunny days." Keep practicing to improve even more!

